Instructing the Architecture Search for Spatial-temporal Sequence Forecasting with LLM

Spatial-temporal sequence forecasting (STSF) is a long-standing research problem with widespread real-world applications. Neural architecture search (NAS), which automates the neural network design, has been shown effective in tackling the STSF problem. However, the existing NAS methods for STSF focus on generating architectures in a time-consuming data-driven fashion, which heavily limits their ability to use background knowledge and explore the complicated search trajectory. Large language models (LLMs) have shown remarkable ability in decision-making with comprehensive internal world knowledge, but how it could benefit NAS for STSF remains unexplored. In this paper, we propose a novel NAS method for STSF based on LLM. Instead of directly generate architectures with LLM, We inspire the LLM's capability with a multi-level enhancement mechanism. Specifically, on the step-level, we decompose the generation task into decision steps with powerful prompt engineering and inspire LLM to serve as instructor for architecture search based on its internal knowledge. On the instance-level, we utilize a one-step tuning framework to quickly evaluate the architecture instance and a memory bank to cumulate knowledge to improve LLM's search ability. On the task-level, we propose a two-stage architecture search, balancing the exploration stage and optimization stage, to reduce the possibility of being trapped in local optima. Extensive experimental results demonstrate that our method can achieve competitive effectiveness with superior efficiency against existing NAS methods for STSF.

==> sections/discussion.tex <==
\section{Limitation}
\label{ch-limitation}

The instability of a large language model will impact the effectiveness and efficiency of the method. The output of the large language model may be entirely different with the exact same input, which creates instability in architecture searching. However, in our experiments, the large average performance of LLaMA-8B shows searching ability with acceptable fluctuation and the future language models with more parameters or better performance may show more stable performance. 

On the other hand, Using the knowledge of a pre-trained large language model and borrowing common knowledge from the history of others is a more effective and efficient way to save efforts for architecture searching to a certain degree. However, the evaluation process for a model in STSF is still time-consuming. Approximate methods with fewer evaluation epochs may work in saving time. In the future, we will focus on the efficiency of evaluating a model. 
